A Calculus for Sensor Networks

We consider the problem of providing a rigorous model for programming wireless sensor networks. Assuming that collisions, packet losses, and errors are dealt with at the lower layers of the protocol stack, we propose a Calculus for Sensor Networks (CSN) that captures the main abstractions for programming applications for this class of devices. Besides providing the syntax and semantics for the calculus, we show its expressiveness by providing implementations for several examples of typical operations on sensor networks. Also included is a detailed discussion of possible extensions to CSN that enable the modeling of other important features of these networks such as sensor state, sampling strategies, and network security.

==> clipboard.tex <==
exemplo com 3 sensores

% \begin{lstlisting}
% MSensor(p) = { deploy = (x) net.deploy[x]; install x }

% MSink(p)   = {}

% M          = {seal = () net.seal[]; install { deploy = () idle } }
% \end{lstlisting}

% such that d(p,p_1) < r but d(p,p_2)> r; d(p_1,p)< r_1 and d(p_1,p_2)<r_1
% and, finally, d(p_2,p_1)< r_2.

% \begin{lstlisting}
% [net.deploy[M]; net.seal[]],MSink(p)] | 
% [idle,MSensor(p_1)] | [idle,MSensor(p_2)] &  d(p,p_1)<r, R-Broadcast \\

% [net.deploy[M]; net.seal[]],MSink(p)] | 
% {[this.deploy[M] || idle, MSensor(p_1)]} | [idle,MSensor(p_2)] & R-Release, S-Monoid-Program \\

% [net.seal[]],MSink(p)] | 
% [this.deploy[M], MSensor(p_1)] | [idle,MSensor(p_2)] & R-Method \\

% [net.seal[]],MSink(p)] | 
% [net.deploy[M]; install M, MSensor(p_1)] | [idle,MSensor(p_2)] & d(p_1,p_2)< r_1, R-Broadcast \\

% [net.seal[]],MSink(p)] | 
% [net.deploy[M]; install M, MSensor(p_1)] {[this.deploy[M] || idle,MSensor(p_2)]} & R-Release \\

% [net.seal[]],MSink(p)] | 
% [install M, MSensor(p_1)] {[net.deploy[M]; install M,MSensor(p_2)]} & R-Release, S-Monoid-Program \\

% [net.seal[]],MSink(p)] | 
% [install M, MSensor(p_1)] | [net.deploy[M]; install M,MSensor(p_2)] & R-Install \\

% [net.seal[]],MSink(p)] | 
% [idle, MSensor(p_1)+M] | [net.deploy[M]; install M,MSensor(p_2)] & **???**  \\

% (como mando fora o net. se nao tiver nada para agregar ? [net. ; P1 ||P2, M] {off} -> [P1||P2,M] ?)

% [net.seal[]],MSink(p)] | 
% [idle, MSensor(p_1)+M] | [install M,MSensor(p_2)] & R-Install \\

% [net.seal[]],MSink(p)] | 
% [idle, MSensor(p_1)+M] | [idle, MSensor(p_2)+M] & d(p,p_1)<r , R-Broadcast \\

% [net.seal[]],MSink(p)] {[this.seal[] || idle, MSensor(p_1)+M]} | 
% [idle, MSensor(p_2)+M] & R-Release, S-Monoid-Program \\

% [idle,MSink(p)] |
% [this.seal[], MSensor(p_1)+M] | [idle, MSensor(p_2)+M] & R-Method \\

% [idle,MSink(p)] | 
% [net.seal[]; install {deploy = () idle}, MSensor(p_1)+M] | 
% [idle, MSensor(p_2)+M] & d(p_1,p_2)<r_1, R-Broadcast \\

% [idle,MSink(p)] | 
% [net.seal[]; install {deploy = () idle}, MSensor(p_1)+M] | 
% {[this.seal[] || idle, MSensor(p_2)+M]} & R-Release, S-Monoid-Program \\

% [idle,MSink(p)] | 
% [install {deploy = () idle}, MSensor(p_1)+M] | 
% [this.seal[], MSensor(p_2)+M] & R-Install \\

% [idle,MSink(p)] | 
% [idle, MSensor(p_1)+M+{deploy = () idle}] | 
% [this.seal[], MSensor(p_2)+M] & R-Method \\

% [idle,MSink(p)] | 
% [idle, MSensor(p_1)+M+{deploy = () idle}] | 
% [net.seal[]; install {deploy = () idle}, MSensor(p_2)+M] & ***???*** \\

% [idle,MSink(p)] | 
% [idle, MSensor(p_1)+M+{deploy = () idle}] | 
% [install {deploy = () idle}, MSensor(p_2)+M] & R-Install \\

% [idle,MSink(p)] | 
% [idle, MSensor(p_1)+M+{deploy = () idle}] | 
% [idle, MSensor(p_2)+M+{deploy = () idle}] &  \\

% \end{lstlisting}


==> fig-tag-oper-semantic.tex <==
\begin{myfigure}
  \begin{gather*}
    \disprule{\Rtrans}
    {
      \frac{
        \dist (p, p') < r_t
      }
      {
        \sensor P M {p'} {r_t'} {r_s'} \parn
        E
        \tagreducesd
        \tagsensor {P \parp \invk {\thisk} {l_i} {\vec v}} M
                   {p'} b {r_t'} {r_s'} {xxxx} \parn
        E
      }
    }
    \\[\rulespace]
    \disprule{\Rtagstructural}
    {
      \frac{
        E_1 \congr E_2 \qquad 
        E_2 \tagreducesd E_3 \qquad
        E_3 \congr E_4
      }
      {
        E_1
        \tagreducesd
        E_4
      }
    }
  \end{gather*}
\caption{Reduction semantics for tagged sensors.}
\label{fig:tag-reduction-semantics}
\end{myfigure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "figsonly"
%%% End: 


==> figsonly.tex <==
%\documentclass{article}
%\usepackage{amsmath, amsthm}
%\usepackage{pdfsync}
%\usepackage{prooftree}

\input{macros}
\begin{document}

% \begin{equation*}
%   \untag(N) =
%   \begin{cases}
%     \sensord, & \text{if } N \text{ is } \tagsensor P M p {r_t}\\
%     \untag(N_1) \parn \untag(N_2), & \text{if } N \text{ is } N_1 \parn N_2\\
%     N, & \text{otherwise}
%   \end{cases}
% \end{equation*}

\begin{equation*}
  E \grmeq N \grmor \tagsensord \grmor E \parn E
\end{equation*}

% Syntax
\input{syntax}
%\input{fig-types}
% Reduction
\input{fig-reduction}

% Type system
%\input{fig-subtype}
%\input{fig-static-val}
%\input{fig-static-ins}
%\input{fig-static-prog}

% Examples
\input{examples}

\vfill\hfill\today
\end{document}

%%% $Id: figsonly.tex,v 1.5 2006/11/24 22:40:39 fmartins Exp $
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> related.tex <==
\section{Related Work}
\label{sec:related}

Here we talk about related work on sensor and wireless networks.



==> syntax-alternativa.tex <==
\begin{myfigure}
\begin{align*}
  & N \grmeq & & \text{\emph{Sensor networks}}\\ 
  & \qquad \;\; \inactionn & & \text{termination}\\
  & \quad \grmor \sensord & & \text{sensor}\\
  & \quad \grmor \Valued & & \text{value}\\
  & \quad \grmor N \parn N & & \text{composition}\\
  \\
  & M \grmeq & & \text{\emph{Modules}}\\ 
  & \qquad \;\; \moduled & & \text{method collection}\\
  \\
  & P \grmeq & & \text{\emph{Programs}}\\ 
  & \qquad \;\; \inactionp & & \text{idle}\\
  & \quad \grmor \newd & & \text{new reference}\\
  & \quad \grmor \invkd & & \text{method invocation}\\
  & \quad \grmor \objd & & \text{object}\\
  & \quad \grmor \defind & & \text{recursive definition}\\
  & \quad \grmor P \parp P & & \text{parallel composition}\\
  & \quad \grmor \installd & & \text{module update} \\
  & \quad \grmor \sensed & & \text{value perception} \\
  & \quad \grmor \ifk\ v\ \thenk\ P\ \elsek\ P & & \text{conditional execution}\\
  \\
  & t \grmeq & & \text{\emph{Targets}}\\ 
  & \qquad \;\; x & & \text{reference}\\
  & \quad \grmor \netk & & \text{broadcast}\\
  & \quad \grmor \thisk & & \text{local}\\
  \\
  & v \grmeq & & \text{\emph{Values}}\\ 
  & \qquad \;\; b & & \text{basic value}\\
  & \quad \grmor l & & \text{label}\\
  & \quad \grmor x & & \text{variable}\\
  & \quad \grmor p & & \text{position}\\
  & \quad \grmor M & & \text{module}\\
%  \\
%  & k \grmeq & & \text{\emph{Kinds}}\\ 
%  & \qquad \;\; m & & \text{measure}\\
%  & \quad \grmor e & & \text{event}
\end{align*}
\caption{Syntax of the sensor calculus.}
\label{fig:syntax-sensor}
\end{myfigure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "figsonly"
%%% End: 


==> syntax.tex <==
\input{fig-syntax}

This section addresses the syntax and the semantics of the Calculus
for Sensor Networks.
%
The syntax of the calculus is given by the grammar in Figure
\ref{fig:syntax-sensor}.
%
The calculus encompasses a two-level structure: \emph{networks} and
\emph{programs}.

% networks
\emph{Networks} $N$ are flat, unstructured collections of
sensors and values.

% Sensors
A sensor $\sensord$ represents an abstraction of a physical
sensing device located at position $p$ and running program $P$.
%
Module $M$ is the collection of methods that the sensor makes
available for internal and for external usage.
%
Typically this collection of methods may be interpreted as the library
of functions of the tiny operating system installed in the sensor.
%
Sensors may only broadcast values to its neighborhood sensors. 
%
Radius $r_t$ defines the transmitting power of a sensor and specifies
the border of communication: a circle centered at position $p$ (the
position of the sensor) with radius $r_t$.
%
Likewise, radius $r_s$ defines the sensing capability of the sensor,
meaning that a sensor may only read values inside the circle centered 
at position $p$ with radius $r_s$.

% values
\emph{Values} $\Valued$ define the field of measures that may be
sensed.
%
A value consists of a tuple $\vec v$ denoting the strength of the
measure at a given position $p$ of the plane.
%
Values are managed by the environment; in CSN there are no primitives
for manipulating values, besides reading (sensing) values.
%
We assume that the environment inserts these values in the network and
update its contents.
%
Networks are combined using the parallel composition operator $\parn$.

% programs
Processes are built from the inactive process $\inactionp$ and from
...
%
%
$\inactionp$ denotes a terminated thread.

and sensing values from the environment $sensed$ th

Programs $P$ and $Q$ may be combined in sequence, $P \seq Q$,
or in parallel, $P \parp Q$.
%
The sequential composition $P \seq Q$ designates a program that first
executes $P$ and then proceeds with the execution of $Q$.
%
In contrast, $P \parp Q$ represents the simultaneous execution of $P$
and $Q$.
%
However we consider that sensors support only a very limited form of
parallelism: $P$ and $Q$ do not interact during their execution; 
%

Mutually recursive method definitions makes possible to represent
infinite behaviours.

% values
\emph{Values} are the data exchanged between sensors, and are basic
values $b$, method labels $l$, positions $p$, and modules $M$.
%
Notice that the calculus in not high-order in the sense that
communication of modules ...

% example
As an example, consider a...

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

